Language Generation via Combinatorial Constraint Satisfaction: A Tree Search Enhanced Monte-Carlo Approach

Generating natural language under complex constraints is a principled formulation towards controllable text generation. We present a framework to allow specification of combinatorial constraints for sentence generation. We propose TSMH, an efficient method to generate high likelihood sentences with respect to a pre-trained language model while satisfying the constraints. Our approach is highly flexible, requires no task-specific training, and leverages efficient constraint satisfaction solving techniques. To better handle the combinatorial constraints, a tree search algorithm is embedded into the proposal process of the Markov chain Monte Carlo (MCMC) to explore candidates that satisfy more constraints. Compared to existing MCMC approaches, our sampling approach has a better mixing performance. Experiments show that TSMH achieves consistent and significant improvement on multiple language generation tasks.

==> plots/5.2.table2-2col.tex <==

\begin{table}[!ht]
\small
\centering
\begin{tabular}{l|l}
\toprule
% Input & waste heat water \\
Keys & waste heat water \\
TSMC & where was the \pink{waste - water heater}? \\
CGMH & what \pink{waste} is there, it seems now? \\
\midrule
% Input & responses protect lungs mechanically \\ 
% & ejecting pathogens respiratory system \\
Keys & responses protect lungs \\
TSMC & what \pink{responses} do your \pink{lungs} have to \pink{protect} you  from pathogenic bacteria? \\
CGMH & how can immune \pink{responses} also occur by not only infecting pathogens in the central nervous system? \\
\midrule
% Input & median temperature winter \\
Keys & median temperature winter \\
TSMC & what is the \pink{median temperature} range in the \pink{winter} months? \\
CGMH & what do you mean we have \pink{median temperature} \pink{winter} and spring, anyways?\\ 
\midrule
% Input & year university warsaw established \\
Keys & university warsaw established \\
TSMC & when was the technical \pink{university} of \pink{warsaw} first formally \pink{established}? \\
CGMH & polish polytechnical institute - \pink{university} of technology \pink{warsaw} - was \pink{established} here in 1964? \\
\midrule
% Input&french catholics concentrated france\\
Keys &catholics concentrated france \\%\midrule
TSMC &why are the french roman \pink{catholics} so densely \pink{concentrated} in southern \pink{france}?\\
CGMH & the \pink{catholics} are now mainly concentrated there. \\
\bottomrule
\multicolumn{2}{c}{(1) Interrogative Sentences} \\ 
\multicolumn{2}{c}{} \\
\toprule
Keys & seat \\ 
TSMC & please get up from your \pink{seat} \\
CGMH& go on in and take your \pink{seat}  \\ \midrule

Keys & careful \\ 
TSMC  & please be so very very \pink{careful}.     \\ 
CGMH& and please be a very very \pink{careful} \\ \midrule

Keys &turn, lights \\
TSMC & \pink{turn} on the lights all the time \\
CGMH & \pink{turn} on near all the main \pink{lights}\\ \midrule

Keys &close, window \\
TSMC& stay \pink{close} enough to the \pink{window}     \\
CGMH& stick \pink{close} enough to meet the \pink{window}     \\ \midrule				
Keys& nice, weekend \\
TSMC&have yourself a very \pink{nice} private \pink{weekend}\\
CGMH& please be \pink{nice} about spending the \pink{weekend}\\ 
\bottomrule
\multicolumn{2}{c}{(2) Imperative Sentences} \\
\end{tabular}
\caption{Case study of generating interrogative and imperative sentences with keywords, where Keys stands for keywords.}\label{tab:case}
\vspace{-0.7cm}
\end{table}

%Our methods can generate sentences which satisfy the grammar rules, while the output from baseline lack completeness.
